Efficient Communication via Self-supervised Information Aggregation for Online and Offline Multi-agent Reinforcement Learning

Utilizing messages from teammates can improve coordination in cooperative Multi-agent Reinforcement Learning (MARL). Previous works typically combine raw messages of teammates with local information as inputs for policy. However, neglecting message aggregation poses significant inefficiency for policy learning. Motivated by recent advances in representation learning, we argue that efficient message aggregation is essential for good coordination in cooperative MARL. In this paper, we propose Multi-Agent communication via Self-supervised Information Aggregation (MASIA), where agents can aggregate the received messages into compact representations with high relevance to augment the local policy. Specifically, we design a permutation invariant message encoder to generate common information-aggregated representation from messages and optimize it via reconstructing and shooting future information in a self-supervised manner. Hence, each agent would utilize the most relevant parts of the aggregated representation for decision-making by a novel message extraction mechanism. Furthermore, considering the potential of offline learning for real-world applications, we build offline benchmarks for multi-agent communication, which is the first as we know. Empirical results demonstrate the superiority of our method in both online and offline settings. We also release the built offline benchmarks in this paper as a testbed for communication ability validation to facilitate further future research.

==> Sections/1_Introduction.tex <==
\section{Introduction}

%考虑引出两部分：
%1. 全局信息global information对多智能体的协同有至关重要的意义；
% 举几个例子，在复杂任务中，人类的团队合作需要全局信息做为支撑，比如大规模的军事对抗中指挥官对全局信息的需求非常迫切。









%2. 当前的marl方法没有良好的运用global information，主流方法均存在问题：
%  1) 隐式通信的ctde类的方法：只在训练时给total q加入state信息，而执行时没有，导致执行时agent只能根据自己的局部观测通过隐式推断global information的方式。但非常明显，每个个体仅利用有限的个体观测信息是非常难在线推断global information的；
%  2) 显示通信的带通信的方法：在训练和执行过程中，考虑通过通信部分裁剪过的信息来实现对global information的推断，但由于来自于多智能体的观测信息是冗余和复杂的，
%3. 
%4. global information比较难以运用，我们采用信息聚合的方式来运用


%说明只通过端到端的训练、只依赖一个单独的环境reward，对ma问题来说无法学到一个好的表示。







% While the end-to-end training method in multi agent learning problem satisfies the simplicity,  which implicitly use the individual’s local observation to infer the global information to achieve coordination, relying on the sole environmental reward signal to learn a representation can aggregate the global information is severly limiting.

 Multi-Agent Reinforcement Learning (MARL)~\cite{cooperativesuvery} has attracted widespread attention \cite{cooperativesuvery, du2021survey} recently, achieving remarkable success in  many complex domains~\cite{canese2021multi},
% Cooperative multi-agent reinforcement learning (MARL) has attracted attention \cite{cooperativesuvery, du2021survey} recently, achieving remarkable success in  many complex domains
such as traffic signal control \cite{du2021multi}, autonomous driving \cite{smarts}, and droplet control \cite{liang2021parallel}. For better coordination on further applications, some issues like non-stationarity~\cite{papoudakis2019dealing}, scalability~\cite{christianos2021scaling} remain to be solved. To solve the non-stationarity caused by the concurrent learning of multiple policies and scalability as the agent number increases, most recent works on MARL adopt the \textit{Centralized Training and Decentralized Execution} (CTDE) \cite{ctde2016, lyu2021contrasting} paradigm, which includes both value-based methods \cite{vdn, qmix2018, qplex, ijcai2022p85} and policy gradient methods \cite{coma, maddpg, dop,ye2022towards}. Under the CTDE paradigm, however, the coordination ability of the learned policies can be fragile due to the partial observability in the multi-agent environment, which is a common challenge in many multi-agent tasks~\cite{mao2020information}. 
While recurrent neural networks could in principle relieve this issue by conditioning the policy on action-observation history \cite{hausknecht2015deep},
% While the recurrent neural network is used to condition policy on action-observation history \cite{hausknecht2015deep},
the uncertainty of other agents (e.g., states and actions) at execution time can result in catastrophic miscoordination and even sub-optimality \cite{ndq,i2c}.

Communication shows great potential in solving these problems~\cite{zaiem2019learning,zhu2022survey}, with which agents can share information such as observations, intentions, or experiences to stabilize the learning process, leading to a better understanding of the environment (or the other agents) and better coordination as a result. Previous communication methods either focus on generating meaningful information~\cite{ndq,kim2020communication,zhang2020succinct} for the message senders, or design techniques such as attention mechanism~\cite{tarmac,niu2021multi}, message gate~\cite{acml,i2c} to filter the most relevant information on raw received messages. These approaches treat the received information as a black box and tacitly assume that policy networks can automatically extract the most critical information from multiple raw messages during policy learning.
% With the only signal given by reinforcement learning, the extraction process may be fairly inefficient, especially in complex scenarios. 
On this occasion, with the only signal given by reinforcement learning, the extraction process may be reasonably inefficient, especially in complex scenarios.
% guided only by the reinforcement learning signal, but it is not very easy in practice, especially in complex scenarios.
% Taking inspiration from self-supervised representation learning in model free reinforcement learning~\cite{ericsson2021self},

% To facilitate the utilization of multiple messages for an efficient communication paradigm. \red{ With the help of widely proven sample efficiency improvement by self-supervised representation learning~\cite{ericsson2021self} in various domains,}
 Motivated by recent advances in state representation learning~\cite{spr, curl}, which reveals that auxiliary representation objectives could facilitate policy learning~\cite{ericsson2021self},
 we aim at efficiently aggregating information as compact representations for policy by designing a novel communication framework \textbf{M}ulti-\textbf{A}gent communication via \textbf{S}elf-supervised \textbf{I}nformation \textbf{A}ggregation (MASIA).
 Specifically, representations are optimized through self-supervised objectives, which encourages the representations to be both abstract of the true states and predictive of the future information. Since agents are guided towards higher cumulative rewards during policy learning, correlating representations with true states and future information could intensify the learning signals in policy learning. In this way, the efficiency of policy learning could be encouraged. Also, considering that permutation invariance of representations can also promote efficiency, we design a self-attention mechanism to maintain the invariance of obtained representations. We also design a network that weighs the aggregated representation for individual agents to derive unique and highly relevant representation to augment local policies.
 % for the message received from multiple teammates under different views, we apply a self-attention mechanism to learn a permutation invariant and member invariant information embedding, which is then optimized to reconstruct the actual state in the centralized training phase.Furthermore, to improve the sample efficiency in \red{low data regimes}, 
 % we extend a strong model-free agent by adding a dynamics model which predicts future latent representations provided by a parameter-wise exponential moving average of the agent itself. 
 % Finally, each agent then learns to extract the most relevant information from the learned aggregated information representation to augment its local policy.
To evaluate our method, we conduct extensive experiments on various cooperative multi-agent benchmarks, including Hallway~\cite{ndq}, Level-Based Foraging~\cite{papoudakis2021benchmarking}, Traffic Junction~\cite{tarmac}, and two maps from StarCraft Multi-Agent Challenge (SMAC)~\cite{ndq}. The experimental results show that MASIA outperforms previous approaches, strong baselines, and ablations of our method.

Our main contributions are:
\begin{itemize}
    \item We propose a novel framework that uses a message aggregation network to extract from multiple messages generated by various teammates, with which we acquire a permutation invariant information aggregation representation. Agents can then use a novel \textit{focusing network} to extract the most relevant information for decision-making.
    % \item We propose a novel framework that fuses information aggregation and information extraction together to provide the most valuable perceptual information for each agent. The information aggregation network is used to generate abstract global information, and the information extraction network extracts individual-relevant information.
    \item Two representation objectives are introduced to make the information representation \textit{compact} and \textit{sufficient}, including the state reconstruction and multi-step future states prediction. 
    \item Sufficient experimental results on various benchmarks and communication conditions demonstrate that our proposed approach significantly improves the communication performance, and visualization results further reveal why it works. % todo by yinh
\end{itemize}


% (guanc)Unlike previous work, we have a few key insights. First, in many application scenarios, the communication bandwidth is sufficient, due to the decentralized nature and partial observability of the multi-agent environment, it is unwise to use local information obtained by only part of the teammates to infer the true state. For instance, several probe robots enter a complex house from different entrances to explore the terrain and search the target. Second, in consideration of the complexity of the multi-agent environment, it is difficult to train multi agent collaboration well with a single environmental reward signal, some self-supervised signals can be designed to assist training by leveraging the complexity of the environment，and RL task can be regarded as a downstream task. Third, agents need to learn to extract the most valuable information for itself from the global information, just as human like to grasp the overall situation above all, and then extract the valuable local part.

==> Sections/2_Problem_Formulation.tex <==
\section{Problem Formulation}
%  This paper considers a fully cooperative multi-agent task with partial observations, which can be modeled as a Dec-POMDP \cite{pomdp}. A Dec-POMDP can be defined by a tuple $\mathcal{M} = \langle \mathcal{N}, \mathcal{S}, \mathcal{A}, P, \Omega, O, R, \gamma \rangle$, where $\mathcal{N} = \{1, \dots, n\}$ is the set of agents, $\mathcal{S}$ is the set of global states, $\mathcal{A}$ is the set of actions, $\Omega$ is the set of observations, and $\gamma \in [0, 1)$ stands for the discounted factor. At each time step, every agent $i \in \mathcal{N}$ can only acquire the observation $o_i\in \Omega$ drawn from the observation function $O(s, i)$ where $s\in \mathcal{S}$, and then choose the action $a_i \in \mathcal{A}$. The joint action $\boldsymbol{a}=\langle a_1, \dots, a_n \rangle$ leads to next state $s'\sim P(s'\mid s, \boldsymbol{a})$ and the global reward $R(s, \boldsymbol{a})$. The formal objective is to find a joint policy $\boldsymbol{\pi}(\boldsymbol{\tau}, \boldsymbol{a})$ to maximize the global value function $Q_{\rm tot}^{\boldsymbol{\pi}}(\boldsymbol{\tau}, \boldsymbol{a}) =\mathbb{E}_{s,\boldsymbol{a} }\left[\sum_{t=0}^\infty\gamma^tR(s, \boldsymbol{a})\mid s_0=s, \boldsymbol{a_0}=\boldsymbol{a}, \boldsymbol{\pi}\right]$. Here, $\boldsymbol{\tau}=\langle \tau_1, \dots, \tau_n \rangle$, and $\tau_i$ represents the history $(o_i^1, a_i^1, \dots, o_i^{t-1}, a_i^{t-1}, o_i^t)$ of agent $i$ at current timestep $t$.


This paper considers a fully cooperative MARL communication problem, which can be modeled as Decentralised Partially Observable Markov Decision Process under Communication (Dec-POMDP-Com)~\cite{pomdp} and formulated as a tuple $\langle \mathcal{N}, \mathcal{S}, \mathcal{A}, P, \Omega, O, R, \gamma , \mathcal{M} \rangle$, where $\mathcal{N} = \{1, \dots, n\}$ is the set of agents, $\mathcal{S}$ is the set of global states, $\mathcal{A}$ is the set of actions, $\Omega$ is the set of observations,  $O$ is the observation function,  $R$ represents the reward function, $\gamma \in [0, 1)$ stands for the discounted factor, and $\mathcal{M}$ indicates the set of message. At each time step, due to partial observability,  each agent $i \in \mathcal{N}$ can only acquire the observation $o_i\in \Omega$ drawn from the observation function $O(s, i)$ with $s\in \mathcal{S}$, each agent 
holds an individual policy $\pi(a_i\mid \tau_i,m_i)$, where $\tau_i$ represents the history $(o_i^1, a_i^1, \dots, o_i^{t-1}, a_i^{t-1}, o_i^t)$ of agent $i$ at current timestep $t$, and $m_i \in \mathcal{M}$ is the message received by the agent $i$. The joint action $\boldsymbol{a}=\langle a_1, \dots, a_n \rangle$ leads to next state $s'\sim P(s'\mid s, \boldsymbol{a})$ and the global reward $R(s, \boldsymbol{a})$. The formal objective is to find a joint policy $\boldsymbol{\pi}(\boldsymbol{\tau}, \boldsymbol{a})$ to maximize the global value function $Q_{\rm tot}^{\boldsymbol{\pi}}(\boldsymbol{\tau}, \boldsymbol{a}) =\mathbb{E}_{s,\boldsymbol{a} }\left[\sum_{t=0}^\infty\gamma^tR(s, \boldsymbol{a})\mid s_0=s, \boldsymbol{a_0}=\boldsymbol{a}, \boldsymbol{\pi}\right]$, with $\boldsymbol{\tau}=\langle \tau_1, \dots, \tau_n \rangle$. As each agent can behave as a message sender as well as a message receiver, this paper considers learning useful message representation in the received end, and agents only use local information $o_i$ as message to share within the team.

We optimize the policy by value-based MARL, where deep Q-learning \cite{mnih2015human} implements the action-value function $Q(s, \boldsymbol{a})$ with a deep neural network $Q(\boldsymbol\tau, \boldsymbol a; \boldsymbol\theta)$ parameterized by $\boldsymbol{\theta}$. This paper follows the CTDE paradigm. In the centralized training phase, deep Q-learning uses a replay memory $\mathcal{D}$ to store the transition tuple $\langle \boldsymbol{\tau}, \boldsymbol{a}, r, \boldsymbol{\tau}^\prime \rangle$. We use $Q(\boldsymbol\tau, \boldsymbol a; \boldsymbol\theta)$ to approximate $Q(s, \boldsymbol a; \boldsymbol\theta)$ to relieve the partial observability. Thus, the parameters $\boldsymbol\theta$ are learnt by minimizing the expected Temporal Difference (TD) error:
 \begin{equation*}
     \mathcal{L}(\boldsymbol{\theta})=\mathbb{E}_{\left(\boldsymbol{\tau}, \boldsymbol{a}, r, \boldsymbol{\tau}^{\prime}\right) \in \mathcal{D}}\left[\left(r+\gamma V\left(\boldsymbol{\tau}^{\prime} ; \boldsymbol{\theta}^{-}\right)-Q(\boldsymbol{\tau}, \boldsymbol{a} ; \boldsymbol{\theta})\right)^{2}\right],
 \end{equation*}
where $V\left(\tau^{\prime} ; \boldsymbol{\theta}^{-}\right)=\max _{\boldsymbol{a}^{\prime}} Q\left(\boldsymbol{\tau}^{\prime}, \boldsymbol{a}^{\prime} ; \boldsymbol{\theta}^{-}\right)$ is the expected future return of the TD target and $\boldsymbol \theta^-$ are parameters of the target network, which will be periodically updated with $\boldsymbol \theta$.

==> Sections/3_Method.tex <==
\section{Method}
\label{sec:method}

\begin{figure}
  \centering
  \includegraphics[width=1\textwidth]{Figure/framework_revision2.pdf}
  \caption{Structure of MASIA. (a) The overall architecture. (b) Information aggregation and extraction. (c) Information aggregation optimization. (d) Transition model learning. }
  \label{fig:framework}
\end{figure}

In this paper, we propose efficient Multi-Agent communication via Self-supervised Information Aggregation (MASIA), a novel multi-agent communication mechanism for promoting cooperation performance. Redundant communications could increase the burden of information processing for each agent to make decisions and pose new challenges for information extraction since plenty of irrelevant information is contained in raw messages. To design an efficient communication mechanism, we believe two properties are of vital importance - \textit{sufficiency} and \textit{compactness}, where sufficiency means a rich amount of information, and compactness calls for higher information density.  
% % When we talk about a \textit{good} communication mechanism in this paper, we hope it \blue{(at least)} has two important properties - \textit{compactness} and \textit{sufficiency}.
% \textit{Compactness} means the received information for each agent should be simple and strongly individual-relevant: it should excludes redundant information and delivers what is most valuable for this specific agent's decision-making; also, we hope the communication messages can be \textit{sufficient}, which means \blue{[@guanc they are extracted from the global information or other information representation, as long as the representation can infer as much information about the global state as possible.Especially when individuals have limited observation, global information cannot be pieced together from individual observation]} they can infer as much information about the global state as possible.

% % 介绍一下我们的算法进行通信的整体流程
% % 介绍一下self-supervised learning设计的部分
% % 介绍一下policy learning设计的部分
% % 介绍一下整体范式

% % To achieve these two requirements above, we design two self-supervised learning tasks and the whole framework of our method is show in Fig.~\ref{fig:framework}. In order to make full use of available information, we let agents broadcast their limited observational information and utilize an encoder shared among agents to transform the observations into representation $z^t$ which is trained 

% To achieve these two requirements above, \blue{[we designed two modules: information aggregation module and information extraction module, as all perceived information are aggregated to generate an information aggregation representation, and then relevant information can be extracted from it. In order to learn a suitable representation]}, we design two self-supervised learning objectives to guide the communication \blue{[representation]} learning and a focusing network to extract most relevant information for each agent. The whole framework of our method is show in Fig.~\ref{fig:framework}. Overall, we let agents broadcast their limited observational information and utilize an encoder shared among agents to transform \blue{[aggregate]} them into a common representation $z^t$. We hope this $z^t$ can restore as much information about the true state as possible (\textit{sufficiency}) and exclude those useless observational features (\textit{compactness}), such as environmental noise in observations. Moreover, as a complete $z^t$ often is not necessary for one specific agent, we let each agent focus on specific parts of $z^t$ (\textit{compactness}).

% following by yinh: 
To meet the standard of sufficiency, a global encoder, which we call Information Aggregation Encoder (IAE), is shared among agents to aggregate the information broadcasted by agents into a common representation. With proper training, this representation could reflect the global observation so that each agent could obtain sufficient information from it to make decisions. As for compactness, we first design an auxiliary loss on the global representation to correlate it with the policy learning process, and make each agent only focus on the part of the representation related to its performance and coordination by the designed focusing network through excluding the unrelated parts. The entire framework of our method is shown in Fig.~\ref{fig:framework}. We introduce the aggregation and extraction process in Sec.~\ref{sec:iae}, and the objectives for compactness and sufficiency in Sec.~\ref{sec:inf rep opt}. Also, a description of the training and execution process flow can be found in Appendix~\ref{apdx:overall flow}.

% which we believe can help to understand our method better

\subsection{Information Aggregation and Extraction} \label{sec:iae}
% In our communication mechanism, we treat the available observational information of each agent as a view of the multi-agent system, and we utilize a shared encoder network to process these information to obtain a representation $z^t$, which called information aggregation representation, and the encoder called information aggregation encoder(IAE). This practice can be seen as a process of \textbf{information aggregation} and we expect the aggregated $z^t$ to be \textit{compact} and \textit{sufficient}. In addition to the algorithmic design for optimizing the aggregation representation which will be detailedly described in Sec.~\ref{sec:inf rep opt}, we apply the self-attention mechanism to build a special information aggregation encoder. As is shown in part (a) of Fig.~\ref{fig:framework}, we firstly perform the self-attention computation for perceived information from all agents: % scripted by yinh: duplicated sentence.
\textbf{Information Aggregation. } Believing that the true state should be reflected from combined messages, we design the aggregation encoder to be capable of subsuming all the messages sent from agents. Also, the communication system in multi-agent systems is flexible and permutation invariant in nature, which calls for a permutation invariant structure for the aggregation encoder. Based on these beliefs, we apply a self-attention mechanism to aggregate multiple messages from different teammates:
\begin{align}
\bm{Q},\bm{K},\bm{V} &= \mathtt{MLP}_{Q,K,V}([o^t_1,\dots,o^t_i,\dots,o^t_n]),\\
\bm{H} &= \mathtt{softmax}(\frac{\bm{Q}\bm{K}^T}{\sqrt{d_k}})\bm{V},
% h^{state} &= \mathtt{pooling}([h_1,\dots,h_j,\dots]),~h_j = \bm{H}_j. 
\end{align}
where the learnable matrices $Q$, $K$, and $V$ transform the perception from all agents into the corresponding query $\bm{Q}$ , key $\bm{K}$, and value $\bm{V}$, which are the concepts defined in the attention mechanism~\cite{vaswani2017attention}.
Specifically, each row vector of $\bm{H}$ can be seen as a querying result of one agent for all available information, and the hidden state $\bm{H}$ will be fed into the subsequent integration network to finally obtain the output aggregated representation $z^t$. A detailed discussion about the design of the integration network can be found in Appendix \ref{implementationdt}. 
\begin{wrapfigure}{r}{0.4\linewidth}
% \vspace*{-5mm}
\centering
\includegraphics[width=\linewidth]{Figure/toy_study.pdf}
% \vspace*{-5mm}
\caption{A toy experiment for information redundancy on the task of Traffic Junction.}
% \vspace*{-6mm}
\label{fig:traffic toy exp}
\end{wrapfigure}
% We claim that the usage of self-attention mechanism can enable a permutation-invariant information processing and enable more flexible and efficient information aggregation for the encoder network.
In the centralized training phase, we use the aggregated representation $z^t$ as extra inputs in addition to the individual observation to feed the value function. Since $z^t$ contains the information required to determine the true state, taking $z^t$ as extra inputs could reduce the uncertainty about the environment states and produce better estimations on the Q-value for value functions under any value-based policy learning algorithm.

% Our approach can be combined with any value-based learning algorithm, and we feed the information aggregation representation $z^t$ above into each agent to help estimate $Q$ function better. This can be interpreted to complement information on the individual limited observation, thus reducing the uncertainty about the environment state when estimating the individual $Q$ function. 
\textbf{Information Extraction. } Similar to the decision process of human beings, global messages are usually redundant for an individual agent to make good coordination in communication systems. 
% However, we claim that the complete information about the global state is not always necessary for each agent's decision-making.
For example, on the task of Traffic Junction~\cite{tarmac}, one natural idea is that the information of neighboring cars are more important for agents to perceive than those distant ones, and the unrelated information in global message may sometimes even confuse the agents and impede the learning when the map is large. A toy experiment shown in Fig.~\ref{fig:traffic toy exp} supports this idea. We apply the QMIX algorithm in Traffic Junction tasks with different sight settings. The results show that the agents learn better policies when in a small-sight setting (sight-1) than both in a super-limited-sight setting (sight-0) and full-sight setting (sight-full).

To make each agent capable of deciding its own perceptive area, we employ the \textbf{focusing network} to weigh the aggregated representations for each agent.
% we make each agent capable of decide to focus on a part of the aggregated information based on its observation,  which can be seen as a process of \textbf{information extraction}. In specific, we feed individual observation $o_i^t$ into a focusing network and obtain a weight vector $w_i^t$ with the same dimension as aggregation representation $z^t$. 
The focusing network is designed as a Multi-Layer Perception (MLP) with the Sigmoid output activation function to ensure that each dimension of $w_i^t$ is bounded between $0$ and $1$. By taking element-wise multiplication with $z^t$, a unique representation could be distilled for individual agents. In this way, if the focusing network produces higher weights on specific dimensions, changes in aggregated representations on these dimensions would be more significant and thus, the agent would be more sensitive to aggregated representation on these parts. On the contrary, if some near-zero weights are outputted on some dimensions, information on those dimensions would be filtered out. In particular, although the information extraction process can, to some extent, reflect the specificity of each agent, we stress the local information by feeding it into the subsequent network together with the extracted representation.

% The weight vector $w_i^t$ is then used to extract information from $z^t$ by doing element-wise multiplication with $z^t$, leading to an individual extracted representation $z_i^t$. Finally, $z_i^t$ and $o_i^t$ are fed together into the subsequent network to estimate the individual $Q$ function. This process works as information extraction because agent can ignore irrelevant features by setting consistent weights near to zero.

\subsection{Information Aggregation Representation Optimization}
\label{sec:inf rep opt}
% Above all, we want the aggregated $z^t$ from observations can express the true global state $s^t$, thus helping alleviate the problem of agents' sub-optimal policy under the limitation of Dec-POMDP in multi-agent reinforcement learning. To achieve this goal, we design an encoder-decoder architecture, which takes agents' collected observational information as input and output an estimation of the global state $\hat{s}^t$. We use the true environment states as supervised labels for decoder and this process exactly resembles the training of an auto-encoder:
As for the learning process of aggregated representation, we consider two typical objectives in global encoder training: reconstruction and multi-step prediction, which constrain the representations produced by the global encoder to be sufficient and compact, respectively. For the reconstruction objective, we employ an additional decoder, which aims to reconstruct the global state by the aggregated representation to allow self-supervision on the global encoder. Specifically, the decoder is optimized together with the aggregation encoder by reconstructing global states $s^t$ from messages $\bm{o}^t$: 
\begin{equation}
    \loss_{ae}(\theta, \eta) = \expect_{\bm{o}^t, s^t} \| g_{\eta}(z^t) - s^t\|^2_2,\quad~z^t = f_{\theta}(\bm{o}^t),~
\end{equation}
where $f_{\theta}, g_{\eta}$ denote the encoder network parameterized by $\theta$ and the decoder network parameterized by $\eta$, respectively. This loss term resembles a classical auto-encoder loss, while the decoder here is not to reconstruct the input, but to recover the global state from representations instead. By utilizing this loss, we guide the encoder to extract observational features that can help infer the global state and let $z^t=f_{\theta}(\bm{o}^t)$ be a sufficient representation.  % yinh: why is it compressed not sufficient 

% Besides, one extra property we expect the latent representation to have is to be predictable, which has been shown effective in some previous works \cite{spr, ericsson2021self}. To equip the aggregated representation $z^t$ with this significant property, 
As for the multi-step prediction objective, we constrain the produced representation to be predictive of future information. Specifically, we design a transition model $h_{\psi}: \mathcal{Z}\times\mathcal{A}^n\rightarrow \mathcal{Z}$ parameterized by $\psi$ as auxiliary model, which predicts the aggregated representation $z^{t+1}$ on next step $t+1$ through the aggregated representation $z^t$ and joint action $\bm{a}^t$ on current step $t$. We regress the predicted aggregated representation after $k$-step rollout on the actual aggregated representation of future messages $\bm{o}^{t+k}$, updating both the aggregation encoder and the auxiliary model via the multi-step prediction loss:
\begin{align}
    \loss_{m}(\theta, \psi) &= \expect_{\bm{o}^t, s^t, \bm{a}^t, \dots, \bm{a}^{t+K-1}, \bm{o}^{t+K}, s^{t+K}}
    \left[\sum_{k=1}^K \|\hat{z}^{t+k} - \Tilde{z}^{t+k}\|_2^2\right],~
    \\ \hat{z}^{t+1} &= h_{\psi}(\Tilde{z}^t, \bm{a}^t),~
    \\ \hat{z}^{t+k} &= h_{\psi}(\hat{z}^{t+k-1},~\bm{a}^{t+k-1}),\quad k=2,\dots,K,
    \\ \Tilde{z}^{t+k} &= f_{\theta}(\bm{o}^{t+k}),\quad k=0,\dots,K.
\end{align}
To further stabilize the learning process, we apply the double network technique, which employs two networks with the same architecture but different update frequencies, for the aggeration encoder. The target network is updated via Exponential Moving Average (EMA) like in SPR~\cite{spr}.
% The target network has the same architecture with the original encoder network and 
%we update the target encoder network via the Exponential Moving Average (EMA) method like in SPR~\cite{spr}.
By forcing the aggregated representation to be predictive of its future states, the aggregated representation could be more correlated with the information required for its decision-making, which meets the compactness standard. Combining these two objectives allows the aggregation encoder to extract more helpful information for agents to coordinate better.
% These two self-supervised learning objectives above can help guide the learning of the encoder network, thus leading the obtained aggregated hidden state to be a compact and sufficient representation of the global state. 
To improve the capability of information extraction on individual agents, we also enhance the learning process of these components with an RL objective. Specifically, we consider minimizing the TD loss:
\begin{equation}
    \loss_{rl}(\theta,\phi) = \mathbb{E}_{\left(\boldsymbol{\tau}, \boldsymbol{a}, r, \boldsymbol{\tau}^{\prime}\right) \in \mathcal{D}}\left[\left(r+\gamma \max_{\boldsymbol{a}^{\prime}}Q_{\rm tot}\left(\boldsymbol{\tau}^{\prime},\boldsymbol{a}^{\prime} ; \theta^{-}, \phi^{-} \right)-Q_{\rm tot}(\boldsymbol{\tau}, \boldsymbol{a} ; \theta, \phi)\right)^{2}\right],~
\end{equation}
where $Q_{\rm tot}$ is computed with individual $Q$-values. The computation of Q-values is actually dependent on the specific value-based learning algorithm. We apply it to prevalent methods, including VDN~\cite{vdn}, QMIX~\cite{qmix2018}, and QPLEX~\cite{qplex}. Moreover, the updating of the focusing network is coupled to the RL objective, making the weights produced by the focusing network could be task-sensitive, which could also facilitate policy learning. 
% we update the focusing network via reinforcement learning signal, which is based on the thought that what information the agent need to focus on should be according to the characteristics of the task.

==> Sections/4_Experiment.tex <==
\section{Experiment}
\label{sec:exp}

We conduct experiments on various benchmarks with different communication request levels\footnote{The codes are available at \href{https://github.com/chenf-ai/MASIA}{https://github.com/chenf-ai/MASIA}}. Specifically, we aim to answer the following questions in this section:  1) How does our method perform when compared with multiple baselines in various scenarios (Sec.~\ref{evaluation of performance})?  2) What kind of knowledge has been learned by the information aggregation encoder (Sec.~\ref{insight of masia})? 3) How can the information extraction module extract the most relevant information for the individual from the learned embedding space (Sec.~\ref{Information Extraction of masia})?  4) Can MASIA be applied to different value decomposition baselines to improve their coordination ability and robustness in various communication conditions (Sec.~\ref{Generality of masia})?
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figure/tot_env.pdf}
	\caption{Multiple benchmarks used in our experiments.}
    % \vspace*{-2mm}
	\label{fig:env}
% 	\vspace*{-2mm}
\end{figure}
\begin{figure}[htbp]
	\centering
	\begin{subfigure}{0.95\linewidth}
	    \centering
	    \includegraphics[width=\linewidth]{Figure/legend.pdf}
	\end{subfigure}
	\begin{subfigure}{\linewidth}
		\centering
    	\begin{subfigure}{0.25\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-hallway-4x6x10-3p_y.pdf}
    	    \caption{Hallway: 4x6x10}
    	\label{fig:hallway_easy}
    	\end{subfigure}
    	\hspace{-0.7em}
    	\begin{subfigure}{0.235\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-Foraging-11x11-6p-4f-s1_.pdf}
    		\caption{LBF: 11x11-6p-4f-s1}
    	\label{fig:lbf_easy}
    	\end{subfigure}
        \hspace{-0.7em}
    	\begin{subfigure}{0.25\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-traffic_junction-10p-14d-0v-medium_.pdf}
    		\caption{\footnotesize{TJ: medium}}
    	\label{fig:traffic_easy}
    	\end{subfigure}
    	\hspace{-0.7em}
    	\begin{subfigure}{0.25\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-1o_10b_vs_1r_.pdf}
    		\caption{SMAC: 1o10b\_vs\_1r}
    	\label{fig:sc2_easy}
    	\end{subfigure}
	\end{subfigure}
	%\qquad
	\begin{subfigure}{\linewidth}
		\centering
    	\begin{subfigure}{0.25\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-hallway-3x5x4x6x10-0x0x1x1x1-5p_y.pdf}
    		\caption{Hallway: 3x5-4x6x10}
    	\label{fig:hallway_hard}
    	\end{subfigure}
    	\hspace{-0.7em}
    	\begin{subfigure}{0.24\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-Foraging-20x20-10p-6f-s1_.pdf}
    		\caption{LBF: 20x20-10p-6f-s1}
    	\label{fig:lbf_hard}
    	\end{subfigure}
    	\hspace{-0.7em}
    	\begin{subfigure}{0.25\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-traffic_junction-20p-18d-0v-hard_.pdf}
    		\caption{TJ: hard}
    	\label{fig:traffic_hard}
    	\end{subfigure}
    	\hspace{-0.7em}
    	\begin{subfigure}{0.25\linewidth}
    		\centering
    		\includegraphics[width=\linewidth]{Figure/exp1-1o_2r_vs_4r_.pdf}
    		\caption{SMAC: 1o2r\_vs\_4r}
    	\label{fig:sc2_hard}
    	\end{subfigure}
	\end{subfigure}
	\caption{Performance comparison with baselines on multiple benchmarks. }
	\label{fig:performance}
\end{figure}
We compare MASIA against a variety of baselines, including communication-free methods and some state-of-the-art communication approaches. QMIX~\cite{qmix2018} is a strong communication-free baseline, and we use the implementation by PyMARL\footnote{Our experiments are all based on the PyMARL framework, which uses SC2.4.6.2.6923.} for comparison, which has shown excellent performance on diverse multi-agent benchmarks \cite{samvelyan2019starcraft}. TarMAC utilizes an attention mechanism to select messages according to their relative importance. The implementation we used is provided by \cite{ndq},
denoted as {TarMAC + QMIX}. NDQ \cite{ndq} aims at learning nearly decomposable Q functions via generating meaningful messages and communication minimization. TMC~\cite{zhang2020succinct} applies a temporal smoothing technique at the message sender end to drastically reduce the amount of information exchanged between agents. For the ablation study, we design a baseline only different in the communication protocol, which adopts a full communication paradigm, where each agent gets message from all other teammates at each timestep, denoted as FullComm.

We evaluate our proposed method on multiple benchmarks shown in Fig.~\ref{fig:env}. Hallway \cite{ndq} is a cooperative environment under partial observability, where $m$ agents are randomly initialized at different positions and required to arrive at the goal $g$ simultaneously. We consider two scenarios with various agents and different groups, and different groups have to arrive at different times. Level Based Foraging (LBF)~\cite{papoudakis2021benchmarking} is another cooperative partially observable grid world game, where agents coordinate to collect food concurrently. Traffic Junction (TJ) \cite{tarmac} is a popular benchmark used to test communication ability, where many cars move along two-way roads with one or more road junctions following the predefined routes, and we test on the medium and hard maps. Two maps named {1o2r\_vs\_4r} and {1o10b\_vs\_1r} from SMAC~\cite{ndq} require the agents to cooperate and communicate to get the position of the enemies. For evaluation, all results are reported with median performance with $95\%$ confidence interval on $5$ random seeds. Details about benchmarks, network architecture and hyper-parameter choices of our method are all presented in Appendices \ref{benchmarkdt}, and \ref{implementationdt}, respectively. 
% Besides, we provide some additional experimental results in Appendix~\ref{ablation}.

\subsection{Communication Performance}
\label{evaluation of performance}
% \subsection{Combination with Value-based Algorithm}
% \begin{figure}[htbp]
% 	\centering
% 	\begin{minipage}{0.69\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{Figure/others/decomposition_compact.pdf}
% 		\caption{Information aggregation visualization, where different colors represent different places at which the entities initialize, the darker the shade, the dot is more close to the end of an episode. For example, type $0$ shows that the enemies initialize at the lower right corner, and our agents initialize on top of them on the map.}
% 		\label{fig:decomposition}
% 	\end{minipage}
% 	%\qquad
% 	\begin{minipage}{0.29\linewidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{Figure/others/heatmap_2.pdf}
% 		\caption{The variations of the agents' weight vectors during an episode, where the horizontal axes indicate the timesteps in an episode, and the vertical axes of the two figures in the middle represent the value for every dimension of the weight vector $w_i^t$. }
% 		\label{fig:visualization_weight}
% 	\end{minipage}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{Figure/others/decomposition.pdf}
%   \caption{Information aggregation visualization, where different colors represent different places at which the entities initialize, the darker the shade, the dot is more close to the end of an episode. For example, type $0$ shows that the enemies initialize at the lower right corner, and our agents initialize on top of them on the map.}
%   \label{fig:decomposition}
% \end{figure}
% Insert text here. Insert text here. Insert text here.
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.9\linewidth]{Figure/tot_visualization_v3.pdf}
  \caption{(a) Information aggregation visualization. Each plotted dot represents an aggregated representation. The three different colors respectively represent three different initialization situations for the enemy entities. For example, type $0$ shows the case when the enemies initialize at the lower right corner. To distinguish aggregated representations on different timesteps, we mark larger timesteps by darker shades of the dots. (b) Visualization of variations of selected agents' focus weight $w_i^t$ in a single episode. We use the horizontal axes for timesteps in one single episode and vertical axes for dimensions of the aggregated representation. The weight is reflected through luminance, and the darker the cell, the larger the weight.
%   Information aggregation visualization, where different colors represent different places at which the entities initialize, the darker shade of a dot implies its closer distance to the end of episode.
  % the darker the shade, the dot is more close to the end of an episode.
%   Type $0$ shows an example of the case when the enemies initialize at the lower right corner, and our agents initialize on top of them on the map. 
  } % yinh: Duplication?
  \label{fig:decomposition}
\end{figure}
We first compare MASIA against multiple baselines to investigate the communication efficiency on various benchmarks. As illustrated in Fig.~\ref{fig:performance}, MASIA achieves the best performance with low variance on all benchmarks, indicating MASIA's strong applicability in scenarios with various difficulties. In Hallway (Fig.~\ref{fig:hallway_easy} \& Fig.~\ref{fig:hallway_hard}), where frequent communications are required for good performance (method without communication such as QMIX fails), other communication methods such as TarMAC, NDQ, and TMC achieve low performance or even fail in this environment. This indicates that inappropriate message generation or message selection would injure the learning process. We believe the reason why FullComm succeeds is that there is hardly any redundancy in agents' observations in Hallway. Our MASIA also succeeds in this environment, showing superiority over others.
% can always learn a policy with good performance since there is hardly any redundant information in agents' observations. Meanwhile, our method MASIA can still take advantage of the information extraction module to help the agents get more self-related information and cooperate better. QMIX fails in Hallway because the agents cannot acquire other agents' positions, indicating the necessity of efficient communication.
The dominating performance of MASIA is even more significant in extended Hallway (Fig.~\ref{fig:hallway_hard}), where agents are separated into different groups. In this environment, MASIA can help agents extract information about their teammates and learn a coordination pattern more efficiently. In LBF (Fig.~\ref{fig:lbf_easy} \& Fig.~\ref{fig:lbf_hard}), existing communication-based MARL methods like NDQ, Fullcomm, and TarMAC struggle due to the sparsity of rewards, especially when the foods are more sparsely distributed (Fig.~\ref{fig:lbf_hard}). In contrast to the performance of QMIX in Hallway, QMIX performs well in LBF, which is attributed to the fact that agents can observe the grids near them, and the mixing network of QMIX can help improve the coordination ability of the fixed group of agents in the training phase. Our method achieves comparable performance with QMIX and TarMAC, showing its strong coordination ability even in sparse reward scenarios. In Traffic Junction (Fig.~\ref{fig:traffic_easy} \& Fig.~\ref{fig:traffic_hard}), TarMAC and NDQ have high variance due to the instability of their messages, while MASIA gains high sample efficiency and can generate steady messages since it aims to reconstruct the state. On the SMAC benchmarks (Fig.~\ref{fig:sc2_easy} \& Fig.~\ref{fig:sc2_hard}), we test on two complex scenarios requiring communication to succeed, where one overseer is in active service to get the information of the enemies. Messages are demanded since the agents have limited sight, so other teammates need the overseer's messages to identify the enemies' positions. 
% \begin{wrapfigure}{r}{0.35\textwidth}
% \vspace*{-5mm}
% \centering
% \includegraphics[width=\linewidth]{Figure/others/heatmap.pdf}
% \vspace*{-6mm}
% \caption{The variations of the agents' weight vectors during an episode, where the horizontal axes indicate the timesteps in an episode, and the vertical axes of the two figures in the middle represent the value for every dimension of the weight vector $w_i^t$. }
% \vspace*{-3mm}
% \label{fig:visualization_weight}
% \end{wrapfigure}
Our method MASIA can maintain the high efficiency of learning and always have competitive performance when converged, which is superior to other baselines.
\subsection{Insights into Information Aggregation Encoder}
\label{insight of masia}
% \red{Show study about IAE: Show the dimensionality reduction visualization and the study about robust Information Aggregation Encoder}
To determine what kind of knowledge the encoder has learned through training, we conduct a visualization analysis on the map {1o2r\_vs\_4r} from SMAC to demonstrate the information contained in the aggregation representation $z^t$. We project the aggregation representation vectors into two-dimensional plane by t-SNE~\cite{van2008visualizing} in Fig~\ref{fig:decomposition}a. We take trajectories from $3$ scenarios of different types of initialization under a task where agents have to seek the enemy at the start, discover the enemy, and finally battle with it for better performance. It can be observed that (1) the aggregated representations could be well distinguished by phases. Projected representations in the seeking phase are far from those in the battle phase and closing phase. This implies that our learned representations could well reflect the true states. (2) the aggregated representations are first divergent in the seeking phase when enemies have been initialized, but become increasingly interlaced later until the closing phase, when enemies have been wiped out after a fierce battle. Since enemies are highly related to decision making, such a result verifies that the aggregated representations exploit also reward information. To sum up, the visualization results show that MASIA can extract valuable global information with these representations.
% yinh: add more details
%这里有几个现象：1）在对通信要求比较高的场景，比如Hallway和sc2上，直接传播o（full comm）往往效果较好，上面复杂的通信结构往往不能根本上提升协作性能，我们的方法几乎与full comm 持平，尤其在Hallway上，更是一马当先；2）在LBF这种不需要通信的场景下，其他通信算法往往
\subsection{Study about Individual Information Extraction}
\label{Information Extraction of masia}
\begin{wrapfigure}{r}{0.3\textwidth}
% \vspace*{-3mm}
\centering
\includegraphics[width=\linewidth]{Figure/exp3-sight_plug_yl.pdf}
% \vspace*{-6mm}
\caption{Performance comparison with varying sights, where s$n$ means the sight range is $n$. }
% \vspace*{-4mm}
\label{fig:agnostic_sights}
\end{wrapfigure}
% \red{Introduce the phenomenon about gate mechanism for extracting features}
% 一方面要介绍学到的关注点都类似，说明我们的方法能帮智能体注意到关键的部分，当两个智能体所处位置基本相同时，他们学到的注意力就全集中在特定部分。
To demonstrate the effectiveness of our information extraction module, we analyze the weights computed by the focusing network. Specifically, we select the TJ (medium) task for evaluation and compare the weights produced by two different agents. In this environment, agents could dynamically enter or leave the plane, making the agents staying in the environment flexible through time. It can be observed that agent $3$ and agent $6$ put focus on similar areas of the aggregated representation. Especially after timestep $15$, when agents $3$ and $6$ are in similar situations and distant from the intersection, their focuses are nearly the same. This verifies that the global state information has been successfully extracted to individual agents. Also, on the top of the figure, we draw a figure to measure the relationship between the cosine similarity of weight vectors of different agents against timesteps. It reveals that the similarity of their focus rises after these two agents begin to proceed in the same line (indicated by the render images posted on the lower parts of Fig.~\ref{fig:decomposition} (b)). This also conforms to the intuition that similar messages should be extracted for similar observations. 
\begin{wrapfigure}{r}{0.3\textwidth}
% \vspace*{-5mm}
\centering
\includegraphics[width=\linewidth]{Figure/exp2-alg_plug_bar.pdf}
% \vspace*{-5mm}
\caption{The increase of winning rates brought about by MASIA on map 1o10b\_vs\_1r.}
% \vspace*{-3mm}
\label{fig:agnostic_methods}
\end{wrapfigure}
\subsection{Generality of Our Method}
\label{Generality of masia}
We aim to verify that the proposed approach is agnostic to various sight ranges and applied value-based MARL methods. We first conduct experiments on the map {1o10b\_vs\_1r} to show that MASIA could also generalize well on agents with limited observations. The results in Sec. \ref{evaluation of performance} show the performance of MASIA when the agents have a sight range of $9$. When we narrow the agents' sight ranges, as shown in Fig.~\ref{fig:agnostic_sights}, by receiving and aggregating messages from teammates, the performance of MASIA does not suffer from a significant drop. Our information aggregation and extraction modules prevent the agent from forfeiting knowledge about the state when the sight range is further limited.

To show the generality of the MASIA framework, we also carry out experiments to integrate MASIA with current baselines, including VDN, QMIX, and QPLEX. As illustrated in Fig.~\ref{fig:agnostic_methods}, when integrated with MASIA, the performance of these baselines can be vastly improved on the map {1o10b\_vs\_1r} from SMAC. In this scenario, one overseer is in service to monitor the enemies. Without communication, the other agents have to search the map for the enemies exhaustively. While with reliable communication, they could communicate with each other and the overseer for better coordination. The results demonstrate that MASIA can efficiently aggregate the messages and improve the agents' coordination ability for these value-based MARL methods. 

==> Sections/5_Related_Work.tex <==
\section{Related Work}
% \subsection{Multi-Agent Communication}
\textbf{Multi-agent reinforcement learning (MARL)}  has made prominent progress these years. Having emerged under the CTDE paradigm, many methods are designed to relieve the non-stationarity issue, and have made noticeable progress these years. Most of them can be roughly divided into policy-based and value-based methods. Typical policy gradient-methods involves MADDPG~\cite{maddpg}, COMA \cite{coma}, MAAC \cite{MAAC}, SQDDPG \cite{sqddpg}, FOP \cite{fop}, and  HAPPO~\cite{kuba2021trust} which explore the optimization of multi-agent policy gradient methods, while value-based methods mainly focus on the factorization of the global value function~\cite{wang2021towards,dou2022understanding}. VDN \cite{vdn} applies a simple additive factorization to decompose the joint value function into agent-wise value functions. 
%  It achieves high flexibility but fails in complex problems. 
QMIX \cite{qmix2018} structurally enforces the learned joint value function to be monotonic to the agent's utilities, which can represent a more affluent class of value functions. QPLEX \cite{qplex} further takes a duplex dueling network architecture to factorize the joint value function, achieving a full expressiveness power of IGM \cite{qtran}. 

% The other category of MARL approaches, on the other hand, mainly concentrates on exploring the optimization of the joint policy. MADDPG \cite{maddpg} implements a centralized critic for each agent and extends the DDPG \cite{lillicrap2015continuous} to multi-agent settings. DOP \cite{dop} combines the merits of multi-agent policy gradient and value factorization from the value-based domain, addressing the issues of centralized-decentralized mismatch and credit assignment for multi-agent coordination. HATPRO and HAPPO~\cite{kuba2021trust} extend the theory of trust region learning to cooperative MARL, and achieve significant performance against strong baselines in multiple benchmarks.

\textbf{Multi-agent Communication} Communication plays a promising role in multi-agent coordination under partial observability~\cite{eccles2019biases,zhu2022survey}. Extensive researches have been made on learning communication protocols to improve performance on cooperative tasks \cite{giles2002learning, foerster2016learning, lazaridou2020emergent, xue2021mis, du2021learning, lin2021learning, DBLP:conf/aaai/YuanWZWZ0Z22, ijcai2022p82}. Previous works can be divided into two categories. One focuses on generating a meaningful message for the message senders. The simplest way is to treat the raw local observation, or the local information history as message \cite{foerster2016learning, communication16}. VBC~\cite{zhang2019efficient} and TMC~\cite{zhang2020succinct} apply techniques, such as variance-based control and temporal smoothing, in the sender end to make the generated messages meaningful and valuable for policy learning. NDQ \cite{ndq} generates minimized messages for different teammates to learn nearly decomposable value functions, and optimize the message generator based on two different information-theory-based regularizers to achieve expressive communication. 
On the contrary, other works try to learn efficiently to extract the most useful message on the receiver end, and they design mechanisms to differentiate the importance of messages. I2C \cite{i2c} and ACML \cite{acml} employ gate mechanism to be selective on received messages. There are also works inspired by the broad application of the attention mechanism \cite{chaudhari2019attentive, de2021attention}.
TarMAC \cite{tarmac} achieves targeted communication via a simple signature-based soft-attention mechanism, where the sender broadcasts a key encoding the properties of the agents, then the receiver attends to all received messages for a weighted sum of messages for decision marking.
SARNet \cite{RangwalaW20} and MAGIC \cite{niu2021multi} further remove the signature in TarMAC and leverage attention-based networks to learn efficient and interpretable relations between entities, decide when and with whom to communicate.

% \subsection{Data-efficient Reinforcement Learning}

% TMC~\cite{zhang2020succinct} applies a temporal smoothing technique to drastically reduce the amount of information exchanged between agents, realizing succinct and robust communication in MARL.
% DIAL \cite{foerster2016learning} is a simple multi-agent communication method trained with reinforcement learning, where agents are able to backpropagate error derivatives through communication channels, which succeeds in simple scenarios such as Switch Riddle. CommNet \cite{communication16} proposes a centralized communication architecture, where the the hidden states of all other agents are collected and averaged to augment local observation. IMAC \cite{wang2020learning} considers the limited-bandwidth communication of multi-agent system, which learns a valuable and compact communication protocol based on the information bottleneck principle. NDQ \cite{ndq} generates minimized messages for different teammates to learn nearly decomposable value functions, and the message is optimized based on two different information-theory-based regularizers, aiming at achieving expressive communication. aiming at achieving expressive communication. TMC \cite{zhang2020succinct} applies a temporal smoothing technique to drastically reduce the amount of information exchanged between agents, achieving succinct and robust communication in MARL. IC3Net \cite{ic3net}, Gated-ACML \cite{acml} utilize gate mechanism to to decide whether a message should be sent.

% using the message to augment the local policy may burden the learning efficiency.

To the best of our knowledge, none of the existing MARL communication methods explicitly consider how the multiple received messages can be optimized for efficient policy learning. Agents may be confused by redundant information from teammates, and simply augmenting the local policy with the raw message may burden the learning. Our proposed method applies a message aggregation module to learn a compact information representation and extracts the most relevant part for decision-making. 

==> Sections/Method-2.tex <==
\begin{algorithm}
	\caption{Model-based State Representation leArning (MSRA)}
	\label{alg}
	\begin{algorithmic}[1]
	   % \REQUIRE Number of Agents $N$,   % 不一定需要
	    \STATE Initialize replay memory $D$
	    \STATE Initialize $Q$ network with random parameters $\theta$
	    \STATE Initialize information aggregation network $f$ with random parameters $\eta$
	    \STATE Initialize VAE encoder with random parameters $\phi$ and decoder with random parameters $\xi$
	    \STATE Initialize latent dynamic model with random parameters $\psi$
	    \STATE Initialize target $Q$ network with parameters $\theta^{-} = \theta$
	    
	    \FOR{$\mbox{episode}=1$ to $M$}
            \STATE Roll-out one trajectory $\bm{\tau}$ with $\epsilon$-greedy policy in the environment
            \STATE Store the trajectory $\bm{\tau}$ in $D$
	        \IF{$|D|$ is larger than batch size $m$}
	            \STATE Sample a minibatch of $m$ trajectories from $D$
	            \STATE Compute the VAE loss:
	                $$
	                    L_{VAE}(\xi,\phi)=\sum_{i=1}^m\sum_{t=1}^T\left[\log p_{\xi}(\bm{s}_i^t|z_i^t) - KL\left(\phi(\bm{s}_i^t)\|\mathcal{N}(0,I)\right)\right],~z_i^t\sim \phi(\bm{s}_i^t)
	                $$
	            \STATE Compute the latent model learning loss:
	                $$
	                    L_{pred}(\phi, \psi)=\sum_{i=1}^m\sum_{t=1}^{T-K}\sum_{k=1}^K\|\tilde{z}_{t+k}-\hat{z}_{t+k}\|^2,
	                $$
	                    where $\tilde{z}_{t+k}$ is the roll-out in latent model, and $\hat{z}_{t+k}$ is $\phi(\bm{s}_i^{t+k})$ with gradient stop operation
	            \STATE Update $\phi, \xi, \psi$ by minimizing $L_{VAE} + \lambda L_{pred}$
	            % learn observation aggregation network
	            \STATE Process the sampled trajectories $[\{(\bm{s}^t_i, \bm{o}^t_i, \bm{u}^t_i, r^t_i, \bm{s}^{t+1}_i)\}_{t=1}^T]_{i=1}^m$ with VAE encoder, and get $[\{(z^t_i, \bm{s}^t_i, \bm{o}^t_i, \bm{u}^t_i, r^t_i, \bm{s}^{t+1}_i)\}_{t=1}^T]_{i=1}^m$ with gradient stop for $\phi$
	            \STATE Update $\eta$ by minimizing the supervised loss:
	            $$
	            L_{supervised}(\eta) = \sum_{i=1}^m\sum_{t=1}^T\left\|f(\bm{o}^t_i) - \bm{z}^t_i\right\|^2.
	            $$
	            % RL update 
	            \STATE Set target $y^t = r^t + \gamma Q_{tot}^{-}(\bm{\tau}^{t+1}, z^{t+1}, \bm{\overline{u}}';\theta^{-}),~ \bm{\overline{u}}'=[\arg\max_{u_i}Q_i^{-}(\bm{\tau}^{t+1}_i, z^{t+1}, u_i;$ $\theta^{-})]_{i=1}^N$
	            \STATE Update $\theta$ by minimizing TD loss:
	            $$
	            L_{TD}(\theta) = \sum_{i=1}^m\sum_{t=1}^{T}\left(Q_{tot}(\bm{\tau}_i^t, z^t_i, \bm{u}_i^t;\theta) - y_i^t\right)^2.
	            $$
	        \ENDIF
	        \STATE Update target network parameters $\theta^{-}=\theta$ with period I
	    \ENDFOR 
    \end{algorithmic}
\end{algorithm}

==> Templates/usage_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Submission of papers to NeurIPS 2021}

% Please read the instructions below carefully and follow them faithfully.

% \subsection{Style}

% Papers to be submitted to NeurIPS 2021 must be prepared according to the
% instructions presented here. Papers may only be up to {\bf nine} pages long,
% including figures. Additional pages \emph{containing only acknowledgments and
% references} are allowed. Papers that exceed the page limit will not be
% reviewed, or in any other way considered for presentation at the conference.

% The margins in 2021 are the same as those in 2007, which allow for $\sim$$15\%$
% more words in the paper compared to earlier years.

% Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
% NeurIPS website as indicated below. Please make sure you use the current files
% and not previous versions. Tweaking the style files may be grounds for
% rejection.

% \subsection{Retrieval of style files}

% The style files for NeurIPS and other conference information are available on
% the World Wide Web at
% \begin{center}
%   \url{http://www.neurips.cc/}
% \end{center}
% The file \verb+neurips_2021.pdf+ contains these instructions and illustrates the
% various formatting requirements your NeurIPS paper must satisfy.

% The only supported style file for NeurIPS 2021 is \verb+neurips_2021.sty+,
% rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
%   Microsoft Word, and RTF are no longer supported!}

% The \LaTeX{} style file contains three optional arguments: \verb+final+, which
% creates a camera-ready copy, \verb+preprint+, which creates a preprint for
% submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
% \verb+natbib+ package for you in case of package clash.

% \paragraph{Preprint option}
% If you wish to post a preprint of your work online, e.g., on arXiv, using the
% NeurIPS style, please use the \verb+preprint+ option. This will create a
% nonanonymized version of your work with the text ``Preprint. Work in progress.''
% in the footer. This version may be distributed as you see fit. Please \textbf{do
%   not} use the \verb+final+ option, which should \textbf{only} be used for
% papers accepted to NeurIPS.

% At submission time, please omit the \verb+final+ and \verb+preprint+
% options. This will anonymize your submission and add line numbers to aid
% review. Please do \emph{not} refer to these line numbers in your paper as they
% will be removed during generation of camera-ready copies.

% The file \verb+neurips_2021.tex+ may be used as a ``shell'' for writing your
% paper. All you have to do is replace the author, title, abstract, and text of
% the paper with your own.

% The formatting instructions contained in these style files are summarized in
% Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

% \section{General formatting instructions}
% \label{gen_inst}

% The text must be confined within a rectangle 5.5~inches (33~picas) wide and
% 9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
% type with a vertical spacing (leading) of 11~points.  Times New Roman is the
% preferred typeface throughout, and will be selected for you by default.
% Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
% indentation.

% The paper title should be 17~point, initial caps/lower case, bold, centered
% between two horizontal rules. The top rule should be 4~points thick and the
% bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
% below the title to rules. All pages should start at 1~inch (6~picas) from the
% top of the page.

% For the final version, authors' names are set in boldface, and each name is
% centered above the corresponding address. The lead author's name is to be listed
% first (left-most), and the co-authors' names (if different address) are set to
% follow. If there is only one co-author, list both author and co-author side by
% side.

% Please pay special attention to the instructions in Section \ref{others}
% regarding figures, tables, acknowledgments, and references.

% \section{Headings: first level}
% \label{headings}

% All headings should be lower case (except for first word and proper nouns),
% flush left, and bold.

% First-level headings should be in 12-point type.

% \subsection{Headings: second level}

% Second-level headings should be in 10-point type.

% \subsubsection{Headings: third level}

% Third-level headings should be in 10-point type.

% \paragraph{Paragraphs}

% There is also a \verb+\paragraph+ command available, which sets the heading in
% bold, flush left, and inline with the text, with the heading followed by 1\,em
% of space.

% \section{Citations, figures, tables, references}
% \label{others}

% These instructions apply to everyone.

% \subsection{Citations within the text}

% The \verb+natbib+ package will be loaded for you by default.  Citations may be
% author/year or numeric, as long as you maintain internal consistency.  As to the
% format of the references themselves, any style is acceptable as long as it is
% used consistently.

% The documentation for \verb+natbib+ may be found at
% \begin{center}
%   \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
% \end{center}
% Of note is the command \verb+\citet+, which produces citations appropriate for
% use in inline text.  For example,
% \begin{verbatim}
%   \citet{hasselmo} investigated\dots
% \end{verbatim}
% produces
% \begin{quote}
%   Hasselmo, et al.\ (1995) investigated\dots
% \end{quote}

% If you wish to load the \verb+natbib+ package with options, you may add the
% following before loading the \verb+neurips_2021+ package:
% \begin{verbatim}
%   \PassOptionsToPackage{options}{natbib}
% \end{verbatim}

% If \verb+natbib+ clashes with another package you load, you can add the optional
% argument \verb+nonatbib+ when loading the style file:
% \begin{verbatim}
%   \usepackage[nonatbib]{neurips_2021}
% \end{verbatim}

% As submission is double blind, refer to your own published work in the third
% person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
% previous work [4].'' If you cite your other papers that are not widely available
% (e.g., a journal paper under review), use anonymous author names in the
% citation, e.g., an author of the form ``A.\ Anonymous.''

% \subsection{Footnotes}

% Footnotes should be used sparingly.  If you do require a footnote, indicate
% footnotes with a number\footnote{Sample of the first footnote.} in the
% text. Place the footnotes at the bottom of the page on which they appear.
% Precede the footnote with a horizontal rule of 2~inches (12~picas).

% Note that footnotes are properly typeset \emph{after} punctuation
% marks.\footnote{As in this example.}

% \subsection{Figures}

% \begin{figure}
%   \centering
%   \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \caption{Sample figure caption.}
% \end{figure}

% All artwork must be neat, clean, and legible. Lines should be dark enough for
% purposes of reproduction. The figure number and caption always appear after the
% figure. Place one line space before the figure caption and one line space after
% the figure. The figure caption should be lower case (except for first word and
% proper nouns); figures are numbered consecutively.

% You may use color figures.  However, it is best for the figure captions and the
% paper body to be legible if the paper is printed in either black/white or in
% color.

% \subsection{Tables}

% All tables must be centered, neat, clean and legible.  The table number and
% title always appear before the table.  See Table~\ref{sample-table}.

% Place one line space before the table title, one line space after the
% table title, and one line space after the table. The table title must
% be lower case (except for first word and proper nouns); tables are
% numbered consecutively.

% Note that publication-quality tables \emph{do not contain vertical rules.} We
% strongly suggest the use of the \verb+booktabs+ package, which allows for
% typesetting high-quality, professional tables:
% \begin{center}
%   \url{https://www.ctan.org/pkg/booktabs}
% \end{center}
% This package was used to typeset Table~\ref{sample-table}.

% \begin{table}
%   \caption{Sample table title}
%   \label{sample-table}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \section{Final instructions}

% Do not change any aspects of the formatting parameters in the style files.  In
% particular, do not modify the width or length of the rectangle the text should
% fit into, and do not change font sizes (except perhaps in the
% \textbf{References} section; see below). Please note that pages should be
% numbered.

% \section{Preparing PDF files}

% Please prepare submission files with paper size ``US Letter,'' and not, for
% example, ``A4.''

% Fonts were the main cause of problems in the past years. Your PDF file must only
% contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
% achieve this.

% \begin{itemize}

% \item You should directly generate PDF files using \verb+pdflatex+.

% \item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
%   menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
%   also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
%   available out-of-the-box on most Linux machines.

% \item The IEEE has recommendations for generating PDF files whose fonts are also
%   acceptable for NeurIPS. Please see
%   \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

% \item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
%   "solid" shapes instead.

% \item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
%   the equivalent AMS Fonts:
% \begin{verbatim}
%   \usepackage{amsfonts}
% \end{verbatim}
% followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
% for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
% workaround for reals, natural and complex:
% \begin{verbatim}
%   \newcommand{\RR}{I\!\!R} %real numbers
%   \newcommand{\Nat}{I\!\!N} %natural numbers
%   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
% \end{verbatim}
% Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

% \end{itemize}

% If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
% you to fix it.

% \subsection{Margins in \LaTeX{}}

% Most of the margin problems come from figures positioned by hand using
% \verb+\special+ or other commands. We suggest using the command
% \verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
% figure width as a multiple of the line width as in the example below:
% \begin{verbatim}
%   \usepackage[pdftex]{graphicx} ...
%   \includegraphics[width=0.8\linewidth]{myfile.pdf}
% \end{verbatim}
% See Section 4.4 in the graphics bundle documentation
% (\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

% A number of width problems arise when \LaTeX{} cannot properly hyphenate a
% line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
% necessary.

% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2021/PaperInformation/FundingDisclosure}.

% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
